A Decision Model for Decentralized Autonomous Organization Platform Selection: Three Industry Case Studies

Decentralized autonomous organizations as a new form of online governance arecollections of smart contracts deployed on a blockchain platform that intercede groupsof people. A growing number of Decentralized Autonomous Organization Platforms,such as Aragon and Colony, have been introduced in the market to facilitate thedevelopment process of such organizations. Selecting the best fitting platform ischallenging for the organizations, as a significant number of decision criteria, such aspopularity, developer availability, governance issues, and consistent documentation ofsuch platforms, should be considered. Additionally, decision-makers at theorganizations are not experts in every domain, so they must continuously acquirevolatile knowledge regarding such platforms and keep themselves updated.Accordingly, a decision model is required to analyze the decision criteria usingsystematic identification and evaluation of potential alternative solutions for adevelopment project. We have developed a theoretical framework to assist softwareengineers with a set of Multi-Criteria Decision-Making problems in software production.This study presents a decision model as a Multi-Criteria Decision-Making problem forthe decentralized autonomous organization platform selection problem. Weconducted three industry case studies in the context of three decentralizedautonomous organizations to evaluate the effectiveness and efficiency of the decisionmodel in assisting decision-makers.

==> name.tex <==
\afterpage{%
\begin{landscape}
\begin{table}[]
\caption{compares a subset of selected studies from the literature that addresses the DAO platform selection problem. The first two columns indicate the selected study (Study) and the publication year (Year).The next column (MCDM) denotes whether the corresponding decision-making technique is an MCDM approach. The next three columns Quality Attribute(QA) determines the type of quality attributes, the data collection type (Data Col.) of the corresponding selected studies, respectively. The sixth column (Approach) indicates the decision-making approach that the studies have employed to address the DAO platform selection problem. the seventh and eighth column indicate research methods (R. Method) (including Expert Interview (Experts), Document Analysis (Doc Analysis), Design Science (Design Sc.), Systematic Literature Review (SLR), Survey, and Case Study) and publication type (Type) (including Research Paper (RP), Master Thesis (MT), and Report (R)), of the corresponding selected studies, respectively. The ninth and tenth and eleventh and twelfth columns(\#F and \#QA and \#C and \#A) signify the number of features and quality attributes and criteria and alternatives considered in the selected studies. The next three columns indicate the numbers of features (\#CF), common quality attributes (\#CQA), and alternatives (\#CA) of this study (the first row) with the selected studies. The last column (Cov.) shows the percentage of the coverage of the considered criteria (quality attributes and features).}
\label{DAO_tableLiterature}
\scriptsize
\centering

\begin{tabular}{|l|r|l|l|l|l|l|l|r|r|r|r|r|r|r|r|}
\hline
\textbf{Study} & \multicolumn{1}{l|}{\textbf{Year}} & \textbf{MCDM} & \textbf{QA} & \textbf{Data Col.} & \textbf{Approach} & \textbf{Research Method} & \textbf{publication type} & \multicolumn{1}{l|}{\textbf{\#F}} & \multicolumn{1}{l|}{\textbf{\#QA}} & \multicolumn{1}{l|}{\textbf{\#C}} & \multicolumn{1}{l|}{\textbf{\#A}} & \multicolumn{1}{l|}{\textbf{\#CF}} & \multicolumn{1}{l|}{\textbf{\#CQA}} & \multicolumn{1}{l|}{\textbf{\#CA}} & \multicolumn{1}{l|}{\textbf{Cov.)}} \\ \hline\hline
Our study & 2021& Yes& \begin{tabular}[c]{@{}l@{}}ISO/IEC 25010\\ Ext. ISO/IEC 9126\end{tabular} & Mixed & DSS& \begin{tabular}[c]{@{}l@{}}Case Study\\ Expert interview\\ Document Analysis\end{tabular} & Research paper & 82 & 46& 128& 28 & 82& 46 & 28& 100\% \\ \hline\hline
\cite{valiente2020evaluating} & 2020& No & Domain specific & Qualitative & Benchmarking & Case Study& Research paper & 9& 2 & 11 & 3& 8 & 2& 3 & 91\%\\ \hline
\cite{liu2020technology}& 2020& No & Domain specific & Qualitative & Benchmarking & Document Analysis & Research paper & 4& 0 & 4& 3& 4 & 0& 3 & 100\% \\ \hline
\cite{ziolkowski2020exploring} & 2020& No & N/A & Qualitative & Benchmarking & \begin{tabular}[c]{@{}l@{}}Document Analysis\\ Expert Interview\end{tabular}& Research paper & 3& 0 & 3& 3& 2 & 0& 2 & 67\%\\ \hline
\cite{lee2020decision} & 2020& Yes& Domain specific & Mixed & AHP& \begin{tabular}[c]{@{}l@{}}Document Analysis\\ Expert Interview\end{tabular}& Research paper & 4& 2 & 6& 3& 4 & 2& 1 & 100\% \\ \hline
\cite{skarzauskiene2020developing} & 2020& No & Domain specific & Qualitative & Benchmarking & Document Analysis & Research paper & 13 & 5 & 18 & 1& 12& 4& 0 & 89\%\\ \hline
\cite{sims2019blockchain} & 2020& No & Domain specific & Quantitative & Benchmarking & Document Analysis & Research paper & 6& 0 & 6& 6& 6 & 0& 2 & 100\% \\ \hline
\cite{faqir2020scalable} & 2020& No & Domain specific & Quantitative& Statistical analysis & Document Analysis & Research paper & 4& 1 & 4& 4 & 4 & 1& 4 & 25\%\\ \hline
\cite{rikken2019governance} & 2019& No & Domain specific & Qualitative & Benchmarking & Expert interview& Research paper & 3& 0 & 3& 1& 2 & 0& 0 & 67\%\\ \hline
\cite{el2020overview} & 2018& No & Domain specific & Quantitative& Statistical analysis & Document Analysis & Research paper & 7& 0 & 7& 4& 1 & 0& 4 & 14\%\\ \hline
\cite{dubeinformation} & 2018& No & Domain specific & Qualitative & Benchmarking & Document Analysis & Research paper & 9& 0 & 9& 1& 2 & 0& 1 & 22\%\\ \hline
\cite{valienteresults} & 2017& No & Domain specific & Qualitative & Benchmarking & \begin{tabular}[c]{@{}l@{}}Document Analysis\\ Case Study\end{tabular}& Research paper & 9& 0 & 9& 3& 8 & 0& 3 & 89\%\\ \hline
\cite{hsieh2018rise}& 2018& Yes& Domain specific & Mixed & Fuzzy& Document Analysis & Dissertation & 9& 4 & 13 & 9& 5 & 3& 0 & 62\%\\ \hline
\cite{dupont2017experiments} & 2017& No & Domain specific & Qualitative & Benchmarking & \begin{tabular}[c]{@{}l@{}}Document Analysis\\ Grounded theory\end{tabular} & Chapter& 2& 0 & 2& 1& 2 & 0& 1 & 100\% \\ \hline
\citeONLINE{tan_2021:Online} & 2020& No & Domain specific & Qualitative & Benchmarking & Document Analysis & Report & 2& 0 & 2& 8& 2 & 0& 2 & 100\% \\ \hline
\cite{Felix_Machart} & 2020& No & Domain specific & Qualitative & Benchmarking & Document Analysis & Report & 8& 0 & 8& 9& 8 & 0& 8 & 100\% \\ \hline
\citeONLINE{DAO_Overview} & 2020& No & Domain specific & Qualitative & Benchmarking & Document Analysis & Report & 9& 0 & 9& 8& 5 & 0& 4 & 56\%\\ \hline
\citeONLINE{George_Samman} & 2020& No & Domain specific & Qualitative & Benchmarking & Document Analysis & Report & 7& 0 & 7& 3& 7 & 0& 10& 100\% \\ \hline
\citeONLINE{Theoryan8:online} & 2019& No & Domain specific & Qualitative & Benchmarking & Document Analysis & Report & 24 & 0 & 24 & 6& 24& 0& 6 & 100\% \\ \hline
\citeONLINE{weller_2019:Online} & 2019& No & Domain specific & Qualitative & Benchmarking & Document Analysis & Report & 8& 0 & 8& 1& 5 & 0& 1 & 63\%\\ \hline
\citeONLINE{noauthor_aragon_nodate:Online} & 2019& No & Domain specific & Qualitative & Benchmarking & Document Analysis & Report & 3& 0 & 3& 4& 2 & 0& 4 & 67\%\\ \hline
& \multicolumn{1}{l|}{} && & && && \multicolumn{1}{l|}{}& \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{}& \multicolumn{1}{l|}{}& \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{}& \multicolumn{1}{l|}{} & 79.24\% \\ \hline
\end{tabular}
\end{table}
\end{landscape}}



==> temp.tex <==

























In literature, some studies employed Benchmarking and Statistical Analysis to evaluate and compare a collection of DAO platforms. 













Katende et al.~\cite{dubeinformation} explore the implications of decentralized autonomous organizations by examining a Blockchain operating system for collective intelligence called DAOStack.This study suggests that although these modern organizations facilitate collaboration and decision-making for directors, it is recommended that directors lean more toward influence-oriented skills as opposed to traditional control-based governance approaches.

This report proposes a working taxonomy of DAOs and looks at relevant industry efforts. It describes DAO and then defines different Forms of DAOs \citeONLINE{binanceresearch_2019:Online}.



Ezra Weller has present the concept and architecture of the DAO stack. This study defines DAOStack as DAOstack is an open-source software stack designed to support a global collaborative network. Organizations built on DAOstack belong in a new category of the structure called DAOs: Decentralized Autonomous Organizations. The stack has been explained, and then use cases of DAOStack, and the first DAO created using DAOStack has been described in this study. The Genesis DAO is the first DAO created using DAOstack, with a mission to advance the DAOstack project and ecosystem \citeONLINE{weller_2019:Online}.

Joshua Tan introduces Govbase in this study. Govbase is organized into three main tables: Projects, Organizations, and Structures. Govbase is organized as a mapping from a list of software projects to a list of governance structures. This report mentioned that if you want to create a DAO, you can query Govbase with ‘DAO,’ and it will return a list of DAO frameworks and introduced eight platforms from Govbase and compared them together~\citeONLINE{tan_2021:Online}. It is different from our study because of the low number of DAO platforms and DAO features observed. Moreover, In Govbase, DAO platforms are introduced, and there are no DAO features for comparison.

This report compares and contrasts four significant ethereum DAO projects' essential approaches, including Aragon, DAOstack, Colony, and Moloch, and attempts to get at their essential points-of-view notable technical innovations which form the basis for their value~\citeONLINE{noauthor_aragon_nodate:Online}.

They have been looking at blockchain and DAO governance from various viewpoints, first elaborating what governance is, what blockchains are in the context of organizational theory, reviewing extant literature (blockchain-focused). In this study, the author presents five DAO frameworks such as Aragon, colony, DAOStack and compares their features. \cite{Felix_Machart}.

This report reviews the various DAOs. DAOs can be thought of as social coordination mechanisms to solve a common goal from a high level. Paired with an on-chain treasury management system responsible for dictating how decisions, funding, and upgrades are made, DAOs provide a technical framework to pool funding securely~\citeONLINE{DAO_Overview}.

This paper aims to identify governance challenges in blockchain applications. This paper has three main contributions. First, they elicit governance challenges in the different forms of blockchain variants. Second, they distinguish various decentralized application types and their specific governance challenges. Third, they classify challenges using various layers and stages of governance in blockchain projects~\cite{rikken2019governance}.

Quinn DuPont describes an emerging form of algorithmic governance, using the case study of ``The DAO'', a short-lived attempt to create a decentralized autonomous organization on the Ethereum blockchain platform~\cite{dupont2017experiments}. The report is a deep dive into the DAO ecosystem, around what DAOs are and their purpose, as well providing an overview of the major current projects~\citeONLINE{DAOADece1:Online}. The purpose of this research is to advance what is currently in play by exploring the essential pre-conditions of DAOs ecosystems through which collective intelligence is Emerging. The exploratory qualitative study evaluated those pre-conditions where communities were able to become more intelligent and identify the main socio-technological obstacles for the emergence of collective intelligence \cite{skarzauskiene2020developing}. 

Faqir-Rhazoui et al. describe DAOHouse, Colony, DAOStack and Aragon and compares some of their feature such as voting system, proposal, scability~\cite{faqir2020scalable}. 



Alexandra Sims shows that business structures have evolved over the centuries, and DAOs are simply another evolution. DAOs require a rethink of the law, including the granting of legal personality to DAOs and granting limited liability to DAO token holders \cite{sims2019blockchain}.

